Rhythmic generation of infinite trees and languages

This work builds on the notion of breadth-first signature of infinite trees and (prefix-closed) languages introduced by the authors in a previous work. We focus here on periodic signatures, a case coming from the study of rational base numeration systems; the language of integer representations in base~$\frac{p}{q}$ has a purely periodic signature whose period is derived from the Christoffel word of slope~$\frac{p}{q}$. Conversely, we characterise languages whose signature are purely periodic as representations of integers in such number systems with non-canonical alphabets of digits.

==> js_beamer4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                           %
%                   js_beamer.tex                           %
%                                                           %
%       Fichier general de macros  ˆ utiliser avec          %
%                   la classe beamer                        %
%                                                           %
%                    040530                                 %
%                                                           %
%                                                           %
%  041203 call \jscolor flag  (for obvious purpose)         %
%                                                           %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\PointTiret}{\quad}
\newcommand{\jscitation}[1]{\ifthenelse{\equal{#1}{}}% \, 
   {}{{\upshape[\textbf{#1}]\hspace*{0.5em}}}}
%
\newcommand{\NomTheorem}{Thm.}
\newcommand{\NomProposition}{Proposition}
\newcommand{\NomRemark}{Remark}
\newcommand{\NomDefinition}{Def.}
\newcommand{\NomFact}{Fact}
\newcommand{\NomProblem}{Problem}
\newcommand{\NomQuestion}{Question}
%
\newtheorem{remark}{\NomRemark}
\newtheorem{proposition}{{\NomProposition}}
\newtheorem{question}{{\NomQuestion}}
\newtheorem{conjecture}{Conjecture}
\newtheorem{observation}{Observation}
% \newtheorem{problem}{{\NomProblem}}
% \newtheorem{fact}{{\NomFact}}
% \newtheorem{definition}{\NomDefinition}
\newcommand{\DE}[2]{%
   \begin{definition}\label{d.#1}{\jscitation{#2}}\PointTiret\ignorespaces}
\newcommand{\DEF}{\end{definition}}
\newcommand{\PR}[2]{\begin{proposition}\label{p.#1}%  
   {\jscitation{#2}}\PointTiret\ignorespaces}
\newcommand{\PRF}{\end{proposition}}
\newcommand{\LE}[2]{\begin{lemma}\label{l.#1}%  
   {\jscitation{#2}}\PointTiret\ignorespaces}
\newcommand{\LEF}{\end{lemma}}
\newcommand{\COR}[2]{\begin{corollary}\label{c.#1}%  
   {\jscitation{#2}}\PointTiret\ignorespaces}
\newcommand{\CORF}{\end{corollary}}
\newcommand{\RE}[1]{\begin{remark}\label{r.#1}%  
   \PointTiret\ignorespaces}
\newcommand{\REF}{\end{remark}}
\renewcommand{\TH}[2]{\begin{theorem}\label{t.#1}% \TH est deja pris dans Latex 2e  
   {\jscitation{#2}}\PointTiret\ignorespaces}
\newcommand{\THF}{\end{theorem}}
%
\newcommand{\FAC}[2]{\begin{fact}\label{fc.#1}%
   {\jscitation{#2}}\PointTiret\ignorespaces}
\newcommand{\FACF}{\end{fact}}
%
\newcommand{\PRO}[2]{\begin{problem}\label{pb.#1}%  
   {\jscitation{#2}}\PointTiret\ignorespaces}
\newcommand{\PROF}{\end{problem}}
%
\newcommand{\QUE}[2]{\begin{question}\label{pb.#1}%  
   {\jscitation{#2}}\PointTiret\ignorespaces}
\newcommand{\QUEF}{\end{question}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% \section{macros de mep}
%  Macros pour la mise en page
%  espaces de lignes negatifs
\newcommand{\bigskipneg}{\vspace*{-5ex}} %960728
\newcommand{\medskipneg}{\vspace*{-2ex}} %960728
\newcommand{\smallskipneg}{\vspace*{-1ex}} %960728
\newcommand{\miniskipneg}{\vspace*{-0.25ex}} %960728
\newcommand{\equskipneg}{\vspace*{-4ex}} %960728
%%%%%% \section{mac. listes}
\newcommand{\jsListe}[1]%
    {\noindent\makebox[\parindent][r]{{\rm (#1)}}\hspace*{.8em}\ignorespaces}
\newcommand{\thi}{\jsListe{i}}
\newcommand{\thii}{\jsListe{ii}}
\newcommand{\thiii}{\jsListe{iii}}
\newcommand{\thiv}{\jsListe{iv}}
\newcommand{\thv}{\jsListe{v}}
\newcommand{\thvi}{\jsListe{vi}}
\newcommand{\thip}{\jsListe{i'}}
\newcommand{\thiip}{\jsListe{ii'}}
\newcommand{\thiiip}{\jsListe{iii'}}
\newcommand{\thivp}{\jsListe{iv'}}
\newcommand{\thvp}{\jsListe{v'}}
\newcommand{\thvip}{\jsListe{vi'}}
\newcommand{\pointn}{\noindent \makebox[1.2em]{$\bullet$}\ignorespaces}
\newcommand{\pointdn}{\makebox[2.4em]{$\bullet$}}
%
\newcommand{\tha}{\jsListe{a}}
\newcommand{\thb}{\jsListe{b}}
\newcommand{\thc}{\jsListe{c}}
\newcommand{\thd}{\jsListe{d}}
\newcommand{\thejs}{\jsListe{e}}
\newcommand{\thf}{\jsListe{f}}
\newcommand{\thg}{\jsListe{g}}
%%%%
\newlength{\HiddenWordWidth}
\newlength{\HWWq}
\newlength{\HWWu}
\newlength{\HWWd}
\newcommand{\NoDim}[2][l]{\makebox[0pt][#1]{\smash{#2}}}
\newcommand{\NoDimMath}[2][c]{\makebox[0pt][#1]{\smash{\SldMath{#2}}}}
\newcommand{\HiddenDimMath}[2][c]{\makebox[\HiddenWordWidth][#1]{$#2$}}
\newcommand{\FixedDimBox}[3][l]%
   {\settowidth{\HiddenWordWidth}{#2}%
    \makebox[\HiddenWordWidth][#1]{#3}}
\newcommand{\FixedDimBoxl}[2]{\FixedDimBox[l]{#1}{#2}}%
\newcommand{\FixedDimBoxc}[2]{\FixedDimBox[c]{#1}{#2}}%
\newcommand{\FixedDimBoxr}[2]{\FixedDimBox[r]{#1}{#2}}%
\newcommand{\HiddenDimBox}[2][l]{\makebox[\HiddenWordWidth][#1]{#2}}
%
\newcommand{\AFDB}[4][c]%
   {%
    \settowidth{\HWWu}{#3}%
    \settowidth{\HWWd}{#4}%
    \ifthenelse{\lengthtest{\HWWu<\HWWd}}%
               {\setlength{\HWWq}{\HWWd}}{\setlength{\HWWq}{\HWWu}}%
    \alt#2{\makebox[\HWWq][#1]{#3}}{\makebox[\HWWq][#1]{#4}}%
   }
%  
\newcommand{\AFDMB}[4][c]%
   {%
    \settowidth{\HWWu}{$#3$}%
    \settowidth{\HWWd}{$#4$}%
    \ifthenelse{\lengthtest{\HWWu<\HWWd}}%
               {\setlength{\HWWq}{\HWWd}}{\setlength{\HWWq}{\HWWu}}%
    \alt#2{\makebox[\HWWq][#1]{$#3$}}{\makebox[\HWWq][#1]{$#4$}}%
   }
%  
\newcommand{\PushLine}{~\hfill~}
% \newcommand{\PushLine}{\hbox{}\hfill\hbox{}}
%
\newcommand{\BmrWait}{\addtocounter{beamerpauses}{1}}
\newcommand{\BmrPass}{\addtocounter{beamerpauses}{-1}}
%
\ifjscolor % 
\newcommand{\mathcolor}{green!40!black}
\newcommand{\ImplColor}{\color{RedOrange}}
\newcommand{\EmphColor}{\color{blue}}
\else
\newcommand{\mathcolor}{black}
\newcommand{\ImplColor}{\color{black}}
\newcommand{\EmphColor}{\color{black}}
\fi 
%
\newcommand{\MathColor}{\color{\mathcolor}}
% 
\newcommand{\SldMath}[1]{{\MathColor $#1$}}
\newcommand{\SldMathSp}[1]{{\MathColor $\msp #1 \msp$}}
\newcommand{\SldMathinMath}[1]{{\MathColor #1}}
\newenvironment<>{SldMathEnv}{\MathColor%
                              \smallskipneg
%                               \smallskipneg%
			      }{%
% 			      \smallskipneg
			      \smallskipneg%
			      }
\newenvironment<>{SldEQ}{\MathColor%
%                          \medskipneg%
			 \begin{equation*}}%
			{\end{equation*}}
% 			 
% 			 \medskipneg}
\newcommand{\SldIff}%
    {{\ImplColor{$\e \pmb{\Longleftrightarrow} \e $}}}
\newcommand{\SldImpl}%
    {{\ImplColor{$\e \pmb{\Longrightarrow} \e $}}}

\newcommand{\emphSld}[1]{{\EmphColor \emph{#1}}}
%
\renewcommand{\CompAuto}[1]%
    {%
     \settodepth{\vbd}{\mbox{$\displaystyle{#1\strut}$}}%
     \settoheight{\vbh}{\mbox{$\displaystyle{#1\strut}$}}%
     \setlength{\vbt}{\vbh}\addtolength{\vbt}{\vbd}%
     {}%
     \psline[linewidth=0.8pt,linecolor=\mathcolor]{c-c}(0,-.65\vbd)(0,.9\vbh)%
     \kern1pt%    
     {#1}%
     \kern1pt%
     \psline[linewidth=0.8pt,linecolor=\mathcolor]{c-c}(0,-.65\vbd)(0,.9\vbh)%
     \kern0.4pt%
     }%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput

==> js_environments3.tex <==
% -*- coding: mac-roman -*-
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%                 js_environments3.tex
%
%   Nouvelle formule : part 2 aprs la dŽfinition des environnements
%
% 091109  reconstruction of a file independant from ETA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%\section{cross-referencing} %%%%%%%%%%%%%%%%%%%
% r\'ef\'erences crois\'ees (entre chapitres diff\'erents)
% 990516 c\'esure pour hyp\'enation
%%%%%%% references to an item  following mnemonic code is used:
%%% 1)  First five letters of the (French) name of the item is used:
%%%        eg  corol  for  corollaire,  exemp  for exemple
%%% 2)  five letters in lower case gives full name,
%%%        capitalised in English only
%%% 3)  first letter in upper case gives abbreviated name,
%%%        capitalised in both English and French
%%% 4)  first letter in upper case, and the five followed by P
%%%        gives abbreviated name (capitalised), followed by the page
%%%        reference
%%% 5)  first TWO letters in upper case, gives full name,
%%%        capitalised in both English and French
%%%
%%%   references listed in alphabetical order
%%%   references have 2 parameters:
%%%     the first one is the chapter ref and is implicitely void,
%%%     for reference call in the same chapter
%%%     the second one is the reference name which is prefixed
%%%     according to the kind of item referenced, which allows to
%%%     give the same name to items of different king and still get
%%%     no confusion.
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  mod. 060813  addition reference to items inside a remark, an 
%%%  example, etc.
\ifenglish
\newcommand{\dex}[1]{\xmd(#1)}
\fi
\iffrench
\newcommand{\dex}[1]{~#1}
\fi
%%%%%%%\subsection{english cross-ref} %%%%%%%%%%%%%%%%%%%
\ifenglish
% 060809 tuning space
\newcommand{\PageRef}[1]{p.\xmd\pageref{#1}}%020422
\newcommand{\PpageRef}[1]{pp.\xmd\pageref{#1}}%040907
\newcommand{\PPageRef}[2]{pp.\xmd\pageref{#1}--\pageref{#2}}%021212
%
\newcommand{\corol}[2][{}]{Corollary~{#1}\ref{c.#2}}%
\newcommand{\COrol}[2][{}]{Corollary~{#1}\ref{c.#2}}%
\newcommand{\Corol}[2][{}]{Cor.~{#1}\ref{c.#2}}
\newcommand{\CorolP}[2][{}]{Cor.~{#1}\ref{c.#2}, \PageRef{c.#2}}
%
\newcommand{\defin}[2][{}]{Definition~{#1}\ref{d.#2}}%
\newcommand{\DEfin}[2][{}]{Definition~{#1}\ref{d.#2}}%
\newcommand{\Defin}[2][{}]{Def.~{#1}\ref{d.#2}}%
\newcommand{\DefinP}[2][{}]{Def.~{#1}\ref{d.#2}, \PageRef{d.#2}}%
%
\newcommand{\equat}[2][{}]{Equation~({#1}\ref{q.#2})}%
\newcommand{\EQuat}[2][{}]{Equation~({#1}\ref{q.#2})}%
\newcommand{\Equat}[2][{}]{Equat.~({#1}\ref{q.#2})}
\newcommand{\EquatP}[2][{}]{Equat.~({#1}\ref{q.#2}), \PageRef{q.#2}}
\newcommand{\equnm}[2][{}]{({#1}\ref{q.#2})\xspace }
\newcommand{\EqunmP}[2][{}]{({#1}\ref{q.#2}), \PageRef{q.#2}}
%%% 060814  for a typo correction in I.6.2.2
\newcommand{\equnmnosp}[2][{}]{({#1}\ref{q.#2})}
%
\newcommand{\exemp}[2][{}]{Example~{#1}\ref{e.#2}}%
\newcommand{\EXemp}[2][{}]{Example~{#1}\ref{e.#2}}%
\newcommand{\Exemp}[2][{}]{Exam.~{#1}\ref{e.#2}}%
\newcommand{\ExempP}[2][{}]{Exam.~{#1}\ref{e.#2}, \PageRef{e.#2}}%
%
\newcommand{\exerc}[2][{}]{Exercise~{#1}\ref{x.#2}}%
\newcommand{\EXerc}[2][{}]{Exercise~{#1}\ref{x.#2}}%
\newcommand{\Exerc}[2][{}]{Exer.~{#1}\ref{x.#2}}
\newcommand{\ExercP}[2][{}]{Exer.~{#1}\ref{x.#2}, \PageRef{x.#2}}
%
\newcommand{\faitxx}[2][{}]{Fact~{#1}\ref{fc.#2}}%??? do not follow
\newcommand{\Fait}[2][{}]{Fact~{#1}\ref{fc.#2}}%
\newcommand{\FaitP}[2][{}]{Fact~{#1}\ref{fc.#2}, \PageRef{fc.#2}}%
%
\newcommand{\figur}[2][{}]{Figure~{#1}\ref{f.#2}}%
\newcommand{\FIgur}[2][{}]{Figure~{#1}\ref{f.#2}}%
\newcommand{\Figur}[2][{}]{Fig.~{#1}\ref{f.#2}}
\newcommand{\FigurP}[2][{}]{Fig.~{#1}\ref{f.#2}, \PageRef{f.#2}}
%
\newcommand{\lemme}[2][{}]{Lemma~{#1}\ref{l.#2}}%
\newcommand{\LEmme}[2][{}]{Lemma~{#1}\ref{l.#2}}%
\newcommand{\Lemme}[2][{}]{Lem.~{#1}\ref{l.#2}}
\newcommand{\LemmeP}[2][{}]{Lem.~{#1}\ref{l.#2}, \PageRef{l.#2}}
%
\newcommand{\nnote}[2][{}]{Note~{#1}\ref{n.#2}}%
\newcommand{\Nnote}[2][{}]{No\-te~{#1}\ref{n.#2}}
\newcommand{\NnoteP}[2][{}]{No\-te~{#1}\ref{n.#2}, \PageRef{n.#2}}
%
\newcommand{\probl}[2][{}]{Problem~{#1}\ref{pb.#2}}%
\newcommand{\Probl}[2][{}]{Prob.~{#1}\ref{x.#2}}%
\newcommand{\ProblP}[2][{}]{Prob.~{#1}\ref{x.#2}, \PageRef{x.#2}}%
%
\newcommand{\propo}[2][{}]{Proposition~{#1}\ref{p.#2}}%
\newcommand{\PRopo}[2][{}]{Proposition~{#1}\ref{p.#2}}%
\newcommand{\Propo}[2][{}]{Prop.~{#1}\ref{p.#2}}
\newcommand{\PropoP}[2][{}]{Prop.~{#1}\ref{p.#2}, \PageRef{p.#2}}
%
\newcommand{\prpri}[2][{}]{Property~{#1}\ref{pp.#2}}%
\newcommand{\PRpri}[2][{}]{Property~{#1}\ref{pp.#2}}%
\newcommand{\Prpri}[2][{}]{Propty~{#1}\ref{pp.#2}}%
\newcommand{\PrpriP}[2][{}]{Propty~{#1}\ref{pp.#2}, \PageRef{pp.#2}}%
\newcommand{\prprs}[2][{}]{Properties~{#1}\ref{pp.#2}}%
%%% 060811 reference to properties with index
\newcommand{\prpridex}[3][{}]{Property~{#1}\ref{pp.#2}\xmd(#3)}%
%
\newcommand{\remar}[2][{}]{Remark~{#1}\ref{r.#2}}%
\newcommand{\Remar}[2][{}]{Rem.~{#1}\ref{r.#2}}
\newcommand{\RemarP}[2][{}]{Rem.~{#1}\ref{r.#2}, \PageRef{r.#2}}
%
\newcommand{\schol}[2][{}]{Scholium~{#1}\ref{sc.#2}}%
\newcommand{\Schol}[2][{}]{Schol.~{#1}\ref{sc.#2}}
%
\newcommand{\theor}[2][{}]{Theorem~{#1}\ref{t.#2}}%
\newcommand{\THeor}[2][{}]{Theorem~{#1}\ref{t.#2}}%
\newcommand{\Theor}[2][{}]{Th.~{#1}\ref{t.#2}}%
\newcommand{\TheorP}[2][{}]{Th.~{#1}\ref{t.#2}, \PageRef{t.#2}}%
%
\newcommand{\jssecti}[2][{}]{Section~{#1}\ref{s.#2}}%
\newcommand{\JSsecti}[2][{}]{Section~{#1}\ref{s.#2}}%
\newcommand{\jsSecti}[2][{}]{Sec.~{#1}\ref{s.#2}}
\newcommand{\jsSectiP}[2][{}]{Sec.~{#1}\ref{s.#2}, \PageRef{s.#2}}
%
\newcommand{\jssubsecti}[2][{}]{Subsection~{#1}\ref{s.#2}}%
%%% \jschap instead of \chap for the latter is used by french.sty
%%% \chap (and not \chapi) as it came from an old version
\newcommand{\jschap}[1]{Chapter~\ref{chap.#1}}%
\newcommand{\jsCHap}[1]{Chapter~\ref{chap.#1}}%
\newcommand{\jsChap}[1]{Chap.~\ref{chap.#1}}
%
\fi
%%%%%%%\subsection{french cross-ref} %%%%%%%%%%%%%%%%%%%
\iffrench
%
\newcommand{\PageRef}[1]{p.\xmd \xmd \pageref{#1}}%020422
\newcommand{\PpageRef}[1]{pp.\xmd \xmd \pageref{#1}}%040907
\newcommand{\PPageRef}[2]{pp.\xmd\xmd\pageref{#1}--\pageref{#2}}%021212
%
\newcommand{\corol}[2][{}]{corollaire~{#1}\ref{c.#2}}%
\newcommand{\COrol}[2][{}]{Corollaire~{#1}\ref{c.#2}}%
\newcommand{\Corol}[2][{}]{Cor.~{#1}\ref{c.#2}}
\newcommand{\CorolP}[2][{}]{Cor.~{#1}\ref{c.#2}, \PageRef{c.#2}}
%
\newcommand{\defin}[2][{}]{d\'e\-fi\-ni\-tion~{#1}\ref{d.#2}}%
\newcommand{\DEfin}[2][{}]{D\'e\-fi\-ni\-tion~{#1}\ref{d.#2}}%
\newcommand{\Defin}[2][{}]{D\'ef.~{#1}\ref{d.#2}}%
\newcommand{\DefinP}[2][{}]{D\'ef.~{#1}\ref{d.#2}, \PageRef{d.#2}}%
%
\newcommand{\equat}[2][{}]{\'e\-qua\-tion~({#1}\ref{q.#2})}%
\newcommand{\EQuat}[2][{}]{\'E\-qua\-tion~({#1}\ref{q.#2})}%
\newcommand{\Equat}[2][{}]{Equat.~({#1}\ref{q.#2})}
\newcommand{\EquatP}[2][{}]{Equat.~({#1}\ref{q.#2}), \PageRef{q.#2}}
\newcommand{\equnm}[2][{}]{({#1}\ref{q.#2})\xspace }
\newcommand{\EqunmP}[2][{}]{({#1}\ref{q.#2}), \PageRef{q.#2}}
%%% 060814  for a typo correction in I.6.2.2
\newcommand{\equnmnosp}[2][{}]{({#1}\ref{q.#2})}
%
\newcommand{\exemp}[2][{}]{exem\-ple~{#1}\ref{e.#2}}%
\newcommand{\EXemp}[2][{}]{Exem\-ple~{#1}\ref{e.#2}}%
\newcommand{\Exemp}[2][{}]{Exem.~{#1}\ref{e.#2}}%
\newcommand{\ExempP}[2][{}]{Exem.~{#1}\ref{e.#2}, \PageRef{e.#2}}%
%
\newcommand{\exerc}[2][{}]{exer\-cice~{#1}\ref{x.#2}}%
\newcommand{\EXerc}[2][{}]{Exer\-cice~{#1}\ref{x.#2}}%
\newcommand{\Exerc}[2][{}]{Exer.~{#1}\ref{x.#2}}
\newcommand{\ExercP}[2][{}]{Exer.~{#1}\ref{x.#2}, \PageRef{x.#2}}
%
\newcommand{\faitxx}[2][{}]{fait~{#1}\ref{fc.#2}}%
\newcommand{\Fait}[2][{}]{Fait~{#1}\ref{fc.#2}}%
\newcommand{\FaitP}[2][{}]{Fait~{#1}\ref{fc.#2}, \PageRef{fc.#2}}%
%
\newcommand{\figur}[2][{}]{fi\-gu\-re~{#1}\ref{f.#2}}%
\newcommand{\FIgur}[2][{}]{Fi\-gu\-re~{#1}\ref{f.#2}}%
\newcommand{\Figur}[2][{}]{Fig.~{#1}\ref{f.#2}}
\newcommand{\FigurP}[2][{}]{Fig.~{#1}\ref{f.#2}, \PageRef{f.#2}}
%
\newcommand{\lemme}[2][{}]{lem\-me~{#1}\ref{l.#2}}%
\newcommand{\LEmme}[2][{}]{Lem\-me~{#1}\ref{l.#2}}%
\newcommand{\Lemme}[2][{}]{Lem.~{#1}\ref{l.#2}}
\newcommand{\LemmeP}[2][{}]{Lem.~{#1}\ref{l.#2}, \PageRef{l.#2}}
%
\newcommand{\nnote}[2][{}]{no\-te~{#1}\ref{n.#2}}%
\newcommand{\Nnote}[2][{}]{No\-te~{#1}\ref{n.#2}}
\newcommand{\NnoteP}[2][{}]{No\-te~{#1}\ref{n.#2}, \PageRef{n.#2}}
%
\newcommand{\probl}[2][{}]{pro\-bl\`eme~{#1}\ref{pb.#2}}%
\newcommand{\Probl}[2][{}]{Prob.~{#1}\ref{x.#2}}%
\newcommand{\ProblP}[2][{}]{Prob.~{#1}\ref{x.#2}, \PageRef{x.#2}}%
%
\newcommand{\propo}[2][{}]{pro\-po\-si\-tion~{#1}\ref{p.#2}}%
\newcommand{\PRopo}[2][{}]{Pro\-po\-si\-tion~{#1}\ref{p.#2}}%
\newcommand{\Propo}[2][{}]{Prop.~{#1}\ref{p.#2}}
\newcommand{\PropoP}[2][{}]{Prop.~{#1}\ref{p.#2}, \PageRef{p.#2}}
%
\newcommand{\prpri}[2][{}]{pro\-pri\'et\'e~{#1}\ref{pp.#2}}%
\newcommand{\PRpri}[2][{}]{Pro\-pri\'et\'e~{#1}\ref{pp.#2}}%
\newcommand{\Prpri}[2][{}]{Propri.~{#1}\ref{pp.#2}}%
\newcommand{\PrpriP}[2][{}]{Propri.~{#1}\ref{pp.#2}, \PageRef{pp.#2}}%
\newcommand{\prprs}[2][{}]{pro\-pri\'et\'es~{#1}\ref{pp.#2}}%
%%% 060811 reference to properties with index
\newcommand{\prpridex}[3][{}]{pro\-pri\'et\'e~{#1}\ref{pp.#2}~#3)}%
%
\newcommand{\remar}[2][{}]{re\-mar\-que~{#1}\ref{r.#2}}%
\newcommand{\Remar}[2][{}]{Rem.~{#1}\ref{r.#2}}
\newcommand{\RemarP}[2][{}]{Rem.~{#1}\ref{r.#2}, \PageRef{r.#2}}
%
\newcommand{\schol}[2][{}]{scho\-lie~{#1}\ref{sc.#2}}%
\newcommand{\Schol}[2][{}]{Schol.~{#1}\ref{sc.#2}}
%
\newcommand{\theor}[2][{}]{th\'eo\-r\`eme~{#1}\ref{t.#2}}%
\newcommand{\THeor}[2][{}]{Th\'eo\-r\`eme~{#1}\ref{t.#2}}%
\newcommand{\Theor}[2][{}]{Th\'eo.~{#1}\ref{t.#2}}%
\newcommand{\TheorP}[2][{}]{Th\'eo.~{#1}\ref{t.#2}, \PageRef{t.#2}}%
%
\newcommand{\jssecti}[2][{}]{sec\-tion~{#1}\ref{s.#2}}%
\newcommand{\JSsecti}[2][{}]{Sec\-tion~{#1}\ref{s.#2}}%
\newcommand{\jsSecti}[2][{}]{Sec.~{#1}\ref{s.#2}}
\newcommand{\jsSectiP}[2][{}]{Sec.~{#1}\ref{s.#2}, \PageRef{s.#2}}
%
\newcommand{\jssubsecti}[2][{}]{sous-sec\-tion~{#1}\ref{s.#2}}%
%%% \jschap instead of \chap for the latter is used by french.sty
%%% \chap (and not \chapi) as it came from an old version
\newcommand{\jschap}[1]{chapitre~\ref{chap.#1}}%
\newcommand{\jsCHap}[1]{Chapitre~\ref{chap.#1}}%
\newcommand{\jsChap}[1]{Chap.~\ref{chap.#1}}
%
\fi
%%%%%%%\subsection{paragraph cross-ref} %%%%%%%%%%%%%%%%%%%
%%% "paragraphe" is more complex for the French and English versions
%%% differ more radically. kept together to witness it more easily
%%%  mod. 040427, 060809 for the space after \S
%%%  mod. 060812  for the command \jsparg
%%%  061116 pas compltement clair. devrait tre plus explicite.
\ifenglish
\newcommand{\jspara}[2][{}]{\S\xmd{#1}\ref{s.#2}}%
\newcommand{\jsparg}[3][{}]{pa\-ra\-graph~{#1}\ref{s.#3}}%
\newcommand{\jsPara}[3][{}]{\S\xmd{#1}\ref{s.#3}} % modifi\'e 040427
\newcommand{\jsParaP}[3][{}]{\S\xmd{#1}\ref{s.#3}, \PageRef{s.#3}} %040427
\fi
\iffrench
\newcommand{\jspara}[2][{}]{pa\-ra\-graphe~{#1}\ref{s.#2}}% 970416
\newcommand{\jsparg}[3][{}]{pa\-ra\-graphe~{#1}\ref{s.#2}~\ref{s.#3}}%
\newcommand{\jsPara}[3][{}]{\S\xmd{#1}\ref{s.#2}~\ref{s.#3}} % 990908
%           % modifi\'e pour faire apparaitre la reference complete
\newcommand{\jsParaP}[3][{}]{\S\xmd{#1}\ref{s.#2}~\ref{s.#3},
                                              \PageRef{s.#3}} %021110
\fi
%%%%%%%%%%%%%%%%%%%%%%%
\endinput
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> js_formating_macros4.tex <==
% -*- coding: mac-roman -*-
%%%%%%%%%%%%%%%%%% js_formating_macros4 %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%
%%%%% 120213  adaptation of the corresponding eta macro file
%%%%%         contains
%%%%%             negative vertical space
%%%%%             pushline
%%%%%             mathematical definition of variable height
%%%%%             two column  macros
%%%%%           no  simplified list
%%%%%           no  reduction of matrices
%%%%%         no ifenglish flag
%%%%%         needs ifdraft flag for the two column macros
%%%%%
%%%%% 130811  addition of
%%%%%              marginal notes
%%%%%         needs ifdraft flag for the NoteDraft macro
%%%%%
%%%%% 131202  version 4 
%%%%%         suppression of
%%%%%              marginal notes (c'est dur de contenter tout le 
%%%%%              monde et son pre)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% \section{negative vertical space}
\newcommand{\bigskipneg}{\vspace*{-5ex}} %960728
\newcommand{\medskipneg}{\vspace*{-2ex}} %960728
\newcommand{\smallskipneg}{\vspace*{-1ex}} %960728
\newcommand{\miniskipneg}{\vspace*{-0.25ex}} %960728
\newcommand{\equskipneg}{\vspace*{-4ex}} %960728
%
\newcommand{\miniskip}{\vspace*{0.1ex}} %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\PushLine}{\hbox{}\hfill\hbox{}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% \section{Mathematical definition}%%%
\newlength{\DefiTest}\setlength{\DefiTest}{0pt}%
\newlength{\DefiHeightu}\newlength{\DefiHeightd}%
\newlength{\DefiDepthu}\newlength{\DefiDepthd}%
\newcommand{\Defi}[2]%
    {%
     \settoheight{\DefiHeightu}{${\displaystyle #1}$}%
     \settodepth{\DefiDepthu}{${\displaystyle #1}$}%
     \addtolength{\DefiHeightu}{\DefiDepthu}%
     \settoheight{\DefiHeightd}{${\displaystyle #2}$}%
     \settodepth{\DefiDepthd}{${\displaystyle #2}$}%
     \addtolength{\DefiHeightd}{\DefiDepthd}%
     \left\{#1%
     \rule[-\DefiDepthd]{\DefiTest}{\DefiHeightd}%
     \xmd\right|%
     \left.%
     \rule[-\DefiDepthu]{\DefiTest}{\DefiHeightu}%
      #2\right\}%
     }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% \section{Twocolumns macros}%%% colonne + figure %%%%%%%%
%%% variables
\newlength{\ColoText}% largeur de la colonne "de texte"
\newlength{\ColoFigu}% largeur de la colonne "de figure"
\newlength{\TextFiguSpace}% intervalle entre les deux colonnes
\newlength{\parindenttemp} % for indentation in minipage
\newlength{\parskiptemp} % for alinea spacing in minioage
\newlength{\fboxseptemp} % pour memoriser \fboxsep
\newcommand{\TFBoxing}{}
\newcommand{\TFVertAlig}{}
\newcommand{\LeftLarg}{}
% values
\setlength{\fboxseptemp}{\fboxsep}% parce qu'on va l'annuler en draft
\setlength{\parindenttemp}{\parindent}
\setlength{\parskiptemp}{\parskip}
\setlength{\TextFiguSpace}{1.2em}% intervalle entre les deux colonnes
\renewcommand{\LeftLarg}{.66}
\ifdraft\renewcommand{\TFBoxing}{\fbox}\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% 3 paramtres
%%% 1) largeur de la colonne de gauche, en % de \textwidth
%%%    valeur implicite : \LeftLarg = 2/3
%%% 2) texte de la colonne de gauche
%%% 3) texte de la colonne de droite (souvent une figure)
%%% Boites alignŽes sur le haut,
%%%        encadrŽes en mode draft
\newcommand{\TxtFg}[3]%
   {%
    \setlength{\ColoText}{#1\textwidth}%
    \setlength{\ColoFigu}{\textwidth}%
    \addtolength{\ColoFigu}{-\ColoText}%
    \addtolength{\ColoText}{-.5\TextFiguSpace}%
    \addtolength{\ColoFigu}{-.5\TextFiguSpace}%
    \ifdraft\setlength{\fboxsep}{0pt}\fi% % mod 000912, 050822
%
    \noi
    \TFBoxing{%
       \begin{minipage}[\TFVertAlig]{\ColoText}%
%           \RstBLS% 050822
          \setlength{\parindent}{\parindenttemp}%
          \setlength{\parskip}{\parskiptemp}%
          \par\vspace*{0mm}% pour l'alignement sur le haut
             #2
       \end{minipage}%
             }%
    \hspace*{\TextFiguSpace}%
    \TFBoxing{%
       \begin{minipage}[\TFVertAlig]{\ColoFigu}%
          \par\vspace*{0mm}%
             #3%
       \end{minipage}%
             }%
%
    \ifdraft\setlength{\fboxsep}{\fboxseptemp}\fi%050822
   }%
%%%
\newcommand{\TextFigu}[3][\LeftLarg]%
   {\renewcommand{\TFVertAlig}{t}\TxtFg{#1}{#2}{#3}}
\newcommand{\TextFiguC}[3][\LeftLarg]%
   {\renewcommand{\TFVertAlig}{c}\TxtFg{#1}{#2}{#3}}
%%%%%%%%% Figures vers l'exterieur avec dŽbordement
%%% ie la colonne "de droite" est du cotŽ de la marge
\newcommand{\TextFiguX}[3][\LeftLarg]
   {%
    \setlength{\ColoText}{#1\textwidth}%
    \setlength{\ColoFigu}{\textwidth}%
    \addtolength{\ColoFigu}{-\ColoText}%
    \addtolength{\ColoText}{-.5\TextFiguSpace}%
    \addtolength{\ColoFigu}{-.5\TextFiguSpace}%
    \addtolength{\ColoFigu}{\ETAExtendedLineWidth}% mod 000912,050822
    \ifdraft\setlength{\fboxsep}{0pt}\fi% % mod 000912, 050822
%
    \noi
    \ifodd\value{page}%
       \TFBoxing{%
          \begin{minipage}[t]{\ColoText}%
             \RstBLS% 050822
             \setlength{\parindent}{\parindenttemp}%
             \setlength{\parskip}{\parskiptemp}%
             \par\vspace*{0mm}% pour l'alignement sur le haut
                #2
          \end{minipage}%
                }%
       \hspace*{\TextFiguSpace}%
       \TFBoxing{%
          \begin{minipage}[t]{\ColoFigu}%
             \par\vspace*{0mm}%
                #3%
          \end{minipage}%
                }%
    \else
       \hspace*{-\ETAExtendedLineWidth}% mod 000912
       \TFBoxing{%
          \begin{minipage}[t]{\ColoFigu}%
             \par\vspace*{0mm}%
                #3%
          \end{minipage}%
                }%
       \hspace*{\TextFiguSpace}%
       \TFBoxing{%
          \begin{minipage}[t]{\ColoText}%
             \RstBLS% 050822
             \setlength{\parindent}{\parindenttemp}%
             \setlength{\parskip}{\parskiptemp}%
             \par\vspace*{0mm}% pour l'alignement sur le haut
                #2
          \end{minipage}%
                }%
    \fi%
    \ifdraft\setlength{\fboxsep}{\fboxseptemp}\fi%050822
   }
%%%%%%%%% 2 colonnes egales
%%% Attention! la dŽnomination est trompeuse
%%% car la colonne de droite ne comporte pas de
%%% retrait. Devrait s'appeler "FiguFigu"
\newcommand{\TextText}[2]{\TextFigu[.5]{#1}{#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%% \subsection{marginal notes}
% \newcommand{\NoteEnMarge}[1]%
%    {%
%     \marginpar[\begin{flushright}%
%                {\sl {\scriptsize #1}}%
%                \end{flushright}]%
%               {\begin{flushleft}%
%                {\sl {\scriptsize #1}}%
%                \end{flushleft}}%
% 	}%
% %%%
% \newcommand{\NoteDraft}[1]{{\ifdraft\NoteEnMarge{#1}\fi}} %030123-050821
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%% \section{enumeration labels} %%%
% %%% simplified version
% \newlength{\retraita}\setlength{\retraita}{1.5\parindent}
% \newlength{\listespa}\setlength{\listespa}{.8em}
% %
% \newcommand{\EnumLbl}[1]{\rm (#1)}%
% \newcommand{\jsListe}[1]%
%     {\noindent\makebox[\retraita][r]{\EnumLbl{#1}}%
%      \hspace*{\listespa}\ignorespaces}
% %
% \newcommand{\tha}{\jsListe{a}}
% \newcommand{\thb}{\jsListe{b}}
% \newcommand{\thc}{\jsListe{c}}
% \newcommand{\thd}{\jsListe{d}}
% \newcommand{\thejs}{\jsListe{e}}
% \newcommand{\thf}{\jsListe{f}}
% \newcommand{\thg}{\jsListe{g}}
% %
% \newcommand{\thi}{\jsListe{i}}
% \newcommand{\thii}{\jsListe{ii}}
% \newcommand{\thiii}{\jsListe{iii}}
% \newcommand{\thiv}{\jsListe{iv}}
% \newcommand{\thv}{\jsListe{v}}
% \newcommand{\thvi}{\jsListe{vi}}
% %
% \newcommand{\thip}{\jsListe{i$'$}}
% \newcommand{\thiip}{\jsListe{ii$'$}}
% \newcommand{\thiiip}{\jsListe{iii$'$}}
% \newcommand{\thivp}{\jsListe{iv$'$}}
% \newcommand{\thvp}{\jsListe{v$'$}}
% \newcommand{\thvip}{\jsListe{vi$'$}}
% %
% \newcommand{\thnu}{\jsListe{1}}
% \newcommand{\thnd}{\jsListe{2}}
% \newcommand{\thnt}{\jsListe{3}}
% \newcommand{\thnq}{\jsListe{4}}
% %%% to be fixed
% \newcommand{\point}{\makebox[\retraita][l]{$\bullet$}}
% \newcommand{\pointr}{\makebox[\retraita][r]{$\bullet$ \ }}
% \newcommand{\pointn}{\noindent \makebox[1.2em]{$\bullet$}\ignorespaces}
%%% liste d'axiomes
% should be followed with a % for a margin of fixed size
% \jspointtiret defined in eta_environments
\newcommand{\Axio}[1]%
   {\pointn #1\hspace*{.1em}\jspointtiret\hspace*{.4em}\ignorespaces}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%\section{matrices}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Mise en page des grosse matrices
% % valeurs des echelles pour eta
% \newcommand{\redmatu}[1]{\scalebox{0.84}{#1}}
% \newcommand{\redmatd}[1]{\scalebox{0.66}{#1}}
% \newcommand{\redmatt}[1]{\scalebox{0.90}{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

